Rank & Sort Loss for Object Detection and Instance Segmentation

We propose Rank & Sort (RS) Loss, a ranking-based loss function to train deep object detection and instance segmentation methods (i.e. visual detectors). RS Loss supervises the classifier, a sub-network of these methods, to rank each positive above all negatives as well as to sort positives among themselves with respect to (wrt.) their localisation qualities (e.g. Intersection-over-Union - IoU). To tackle the non-differentiable nature of ranking and sorting, we reformulate the incorporation of error-driven update with backpropagation as Identity Update, which enables us to model our novel sorting error among positives. With RS Loss, we significantly simplify training: (i) Thanks to our sorting objective, the positives are prioritized by the classifier without an additional auxiliary head (e.g. for centerness, IoU, mask-IoU), (ii) due to its ranking-based nature, RS Loss is robust to class imbalance, and thus, no sampling heuristic is required, and (iii) we address the multi-task nature of visual detectors using tuning-free task-balancing coefficients. Using RS Loss, we train seven diverse visual detectors only by tuning the learning rate, and show that it consistently outperforms baselines: e.g. our RS Loss improves (i) Faster R-CNN by ~ 3 box AP and aLRP Loss (ranking-based baseline) by ~ 2 box AP on COCO dataset, (ii) Mask R-CNN with repeat factor sampling (RFS) by 3.5 mask AP (~ 7 AP for rare classes) on LVIS dataset; and also outperforms all counterparts. Code is available at: https://github.com/kemaloksuz/RankSortLoss

==> RankSort (arXiv)/sections/1.Introduction.tex <==
\section{Introduction}
\label{sec:Intro}
\begin{figure}
    \centerline{
        \includegraphics[width=0.48\textwidth]{figures/Teaser.pdf}
    }
    \caption{A ranking-based classification loss vs RS Loss. %(a) A generic visual detection pipeline includes many heads from possibly multiple stages. %Mask head is used for instance segmentation and commonly an auxiliary head An auxiliary head, in addition to the standard ones, is common in recent methods (e.g. centerness head for ATSS \cite{ATSS}, IoU head for PAA \cite{paa} and mask IoU head for Mask-scoring R-CNN \cite{maskscoring}). Such heads help learn localization quality and prioritize examples during inference (e.g. by multiplying classification scores by the predicted localisation quality). Sampling heuristics are also common to ensure balanced training. Such architectures require many hyper-parameters and are delicate to tune. 
    (a) Enforcing to rank positives above negatives provides a useful objective for training, however, it ignores ordering among positives. (b) Our RS Loss, in addition to raking positives above negatives, aims to sort positives wrt. their continuous IoUs (positives: a green tone based on its label, negatives: orange).  We propose  Identity Update (Section \ref{sec:IdentityUpdate}), a reformulation of  error-driven update with backpropagation, to tackle these ranking and sorting operations which are difficult to optimize due to their non-differentiable nature. %(both in dashed boxes in (a)) and still outperform baseline networks. 
    %(c) We analyze several design choices and show that RS Loss can be combined by localization losses which are simply balanced based on loss values, requiring no tuning different from lambdas, thereby further simplifying training pipelines. Gradients are computed using bold variables, normal font indicates scalers.
    \label{fig:Teaser}
} 
\end{figure}

Owing to their multi-task (e.g. classification, box regression, mask prediction) nature, object detection and instance segmentation methods rely on  loss functions of the form:
%
\begin{align}
    \label{eq:LossVisualDetection}
    \mathcal{L}_{VD}= \sum \limits_{k \in \mathcal{K}} \sum \limits_{t \in \mathcal{T}} \lambda_{t}^k \mathcal{L}_{t}^k,
\end{align}
%
which combines $\mathcal{L}_{t}^k$, the loss function for  task $t$ on stage $k$ (e.g. $|\mathcal{K}|=2$ for Faster R-CNN \cite{FasterRCNN} with RPN and R-CNN), weighted by a hyper-parameter $\lambda_{t}^k$. In such formulations, the number of hyper-parameters can easily exceed 10 \cite{aLRPLoss}, with additional hyper-parameters arising from  task-specific imbalance problems \cite{Review}, e.g. the positive-negative imbalance in the classification task, and if a cascaded architecture  is used (e.g. HTC \cite{HTC} employs $3$ R-CNNs with different $\lambda_{t}^k$). Thus, although such loss functions have led to unprecedented successes, they require tuning, which is time consuming, leads to sub-optimal solutions and makes fair comparison of methods challenging. 

%(ii) Such formulations ignore correlation between the tasks \cite{aLRPLoss}, failing to provide e.g. high-quality localisation for high-quality predictions.

%Tuning hyper-parameters in the loss functions of visual detection tasks (e.g. object detection, instance segmentation) is challenging mainly due to (i) their multi-task nature (e.g. classification, box regression and mask learning tasks in instance segmentation \cite{MaskRCNN,yolact}) and (ii) in some cases, multi-stage design (e.g. four detectors, comprising one RPN \cite{FasterRCNN} and three Fast R-CNNs \cite{FastRCNN}, are trained within Cascade R-CNN \cite{CascadeRCNN}). Furthermore, task-specific imbalance problems \cite{Review}, such as the positive-negative imbalance (a.k.a. class imbalance) in the classification task, can require more hyper-parameters, degrading the severity of this challenge and, in some cases, ending up with more than 10 hyperparameters to be tuned together \cite{aLRPLoss}.

Recently proposed \textit{ranking-based} loss functions, namely ``Average Precision (AP) Loss'' \cite{APLoss} and ``average Localisation Recall Precision (aLRP) Loss'' \cite{aLRPLoss}, offer two important advantages over the classical \textit{score-based} functions (e.g. Cross-entropy Loss and Focal Loss \cite{FocalLoss}): (1) They directly optimize the performance measure (e.g. AP), thereby providing consistency between training and evaluation objectives. This also reduces the number of hyper-parameters as the performance measure (e.g. AP) does not typically have any hyper-parameters. (2) They are robust to class-imbalance due to their ranking-based error definition.  Although these losses have yielded state-of-the-art (SOTA)  performances, they need longer training and more augmentation. %, thus, have not been commonly adopted yet.

Broadly speaking, the ranking-based losses (AP Loss and aLRP Loss) focus on ranking positive examples over negatives, but %they ignore any kind of interaction among positives
they do not explicitly model positive-to-positive interactions. However, there is evidence that it is helpful to prioritize predictions wrt. their localisation qualities by using an auxiliary (aux. - e.g. IoU, centerness) head \cite{IoUNet,FCOS,ATSS,paa} or by supervising the classifier to directly regress IoUs of the predictions without an aux. head (as  shown by Li et al. \cite{GFL} in Quality Focal Loss - QFL).
%thanks to discarding their inconsistency as they are trained only with positives but tested on all examples.

%prioritizing  predictions wrt. their IoUs has  a positive effect on the final performance. Istersen burada "prioritizing  predictions wrt. their IoUs" faydali oldugu eskiden beri biliniyordu \cite{aux head ve IoU regress calismalari} diyebiliriz. 


In this paper, we propose Rank \& Sort (RS) Loss as a ranking-based loss function to train visual detection (VD -- i.e. object detection and instance segmentation) methods. RS Loss not only ranks positives above negatives (Fig. \ref{fig:Teaser}(a)) but also sorts positives among themselves with respect to their continuous IoU values (Fig. \ref{fig:Teaser}(b)). This approach brings in several crucial benefits. Due to the prioritization of positives during training, detectors trained with RS Loss do not need an aux. head, and due to its ranking-based nature, RS Loss can handle extremely imbalanced data (e.g. object detection \cite{Review}) without any sampling heuristics. Besides, except for the learning rate, RS Loss does not need any hyper-parameter tuning thanks to our tuning-free task-balancing coefficients. Owing to this significant simplification of training, we can apply RS Loss to different methods (i.e. multi-stage, one-stage, anchor-based, anchor-free) easily (i.e. \textit{only by tuning the learning rate}) and demonstrate that RS Loss consistently outperforms baselines. 

Our contributions can be summarized as follows: 

\noindent \textbf{(1)} We reformulate the incorporation of error-driven optimization into backpropagation to optimize non-differentiable ranking-based losses as \textit{Identity Update}, which uniquely provides interpretable loss values during training and allows definition of intra-class errors (e.g. the sorting error among positives). 

\noindent \textbf{(2)} We propose \textit{Rank \& Sort Loss} that defines a ranking objective between positives and negatives as well as a sorting objective to prioritize positives wrt. their continuous IoUs. Due to this ranking-based nature, RS Loss can  train  models in the presence of highly imbalanced data. 

\noindent \textbf{(3)} We present the effectiveness of RS Loss on a diverse set of four object detectors and three instance segmentation methods only by tuning the learning rate and without any aux. heads or sampling heuristics on the widely-used COCO and long-tailed LVIS benchmarks: E.g. (i) Our RS-R-CNN improves Faster-CNN by $\smallsim3$ box AP on COCO, (ii) our RS-Mask R-CNN improves repeat factor sampling by $\smallsim3.5$ mask AP ($\smallsim7$ AP for rare classes) on LVIS.
%, (iii) our RS-YOLACT improves YOLACT by more than $3$ box AP and $\smallsim1.5$ mask AP.
%e.g. RS Loss improves Mask R-CNN by $+2.0$ mask and box APs, yielding better performance than Mask-scoring R-CNN with an auxiliary mask IoU head.


%Recently proposed \textit{ranking-based} loss functions, Average Precision (AP) Loss \cite{APLoss} and average Localisation Recall Precision (aLRP) Loss \cite{aLRPLoss}, are (i) simple-to-tune since they directly optimize performance measures without introducing several hyper-parameters, and (ii) robust to class imbalance owing to their ranking-based error definition, also consistent with performance evaluation, which penalizes predictions only when the positives are not ranked above the negatives during training. A drawback is that they require longer training and more augmentation, thus, have not been commonly adopted yet. Therefore, despite these advantages, the \textit{score-based} alternatives (e.g. Cross-entropy Loss and Focal Loss \cite{FocalLoss}) still prevail. 

%Recently, Li et al. \cite{GFL} introduced Quality Focal Loss (QFL), a score-based loss function that is robust to class imbalance and uses IoU between a prediction and ground truth as a continuous label (i.e. between $0$ and $1$). Directly supervising the classifier to regress these IoUs with QFL allows removing the auxiliary (e.g. centerness, IoU) head of one-stage detectors \cite{ATSS,FCOS}, designed for the same regression purpose, and also improves the performance thanks to discarding the inconsistency of auxiliary heads as they are trained only with positives but tested on all examples. Thus, with QFL, the classifier prioritizes predictions wrt. IoUs, which has a positive effect on Non-Maximum-Suppression (NMS) \cite{GFL} and the computation of AP \cite{aLRPLoss}.

==> RankSort (arXiv)/sections/2.RelatedWork.tex <==
\section{Related Work}
\textbf{Auxiliary heads and continuous labels.} Predicting the localisation quality of a detection with an aux. centerness \cite{FCOS,ATSS}, IoU \cite{IoUNet,paa}, mask IoU \cite{maskscoring} or uncertainty head \cite{KLLoss} and combining these predictions with the classification scores for NMS are shown to improve detection performance.  Lin et al. \cite{GFL} discovered  that using continuous IoUs of predictions to supervise the classifier outperforms using an aux. head. Currently, Lin et al.'s ``Quality Focal Loss'' \cite{GFL} is the only method that is robust to class imbalance \cite{Review} and uses continuous labels to train the classifier. With RS Loss, we investigate the generalizability of this idea on different networks (e.g. multi-stage networks \cite{FasterRCNN,CascadeRCNN}) and on a different task (i.e. instance segmentation). % by using our ranking-based RS Loss.

\textbf{Ranking-based losses in VD}. Despite their advantages,  ranking-based losses are  non-differentiable and difficult to optimize. To address this challenge, black-box solvers \cite{RankBasedBlackboxDifferentiation} use an interpolated AP surface, though yielding little gain in object detection. DR Loss \cite{DRLoss} achieves ranking between positives and negatives by enforcing a margin with Hinge Loss. Finally, AP Loss \cite{APLoss} and aLRP Loss \cite{aLRPLoss} optimize the performance metrics, AP and LRP \cite{LRP} respectively, by using the error-driven update of perceptron learning \cite{Rosenblatt} for the non-differentiable parts. However, they need longer training and heavy augmentation. The main difference of RS Loss is that it also considers continuous localisation qualities as labels.

\textbf{Objective imbalance in VD}. The common strategy in VD is to use $\lambda_t^k$ (Eq. \ref{eq:LossVisualDetection}), a scalar multiplier, on each task and tune them by grid search \cite{paa,yolact}. Recently, Oksuz et al. \cite{aLRPLoss} employed a self-balancing strategy to balance classification and box regression heads, both of which compete for the bounded range of aLRP Loss. Similarly, Chen et al. \cite{SamplingHeuristics} use the ratio of classification and regression losses to balance these tasks. In our design, each loss $\mathcal{L}_t^k$ for a specific head has its own bounded range and thus, no competition ensues among heads. Besides, we use $\mathcal{L}_t^k$s with similar ranges, and  show that our RS Loss can simply be combined with a simple task balancing strategy based on loss values, and hence does not require any tuning except the learning rate.



==> RankSort (arXiv)/sections/3.IdentityUpdate.tex <==
\section{Identity Update for Ranking-based Losses}
\label{sec:IdentityUpdate}
Using a ranking-based loss function is attractive thanks to its compatibility with common performance measures (e.g. AP). It is challenging, however, due to the non-differentiable nature of ranking. Here, we first revisit an existing solution \cite{APLoss,aLRPLoss} that overcomes this non-differentiability by incorporating error-driven update \cite{Rosenblatt} into backpropagation (Section \ref{subsec:Errordriven}), and then present our reformulation (Section \ref{subsec:IdentityUpdate}), which uniquely (i) provides interpretable loss values and (ii) takes into account intra-class errors, which is crucial for using continuous labels.

\begin{figure}
    \centerline{
        \includegraphics[width=0.48\textwidth]{figures/IdentityUpdate.pdf}
    }
    \caption{Three-step computation (green arrows) and optimization (orange arrows) algorithms of ranking-based loss functions. Our identity update (i) yields interpretable loss values (see Appendix \ref{sec:RSLossDetails} for an example on our RS Loss), (ii) replaces Eq. \ref{eq:GeneralPrimaryTermDefinition} of previous work \cite{aLRPLoss} by Eq. \ref{eq:PrimaryTermIdentityUpdate} (green arrow in Step 2) to allow intra-class errors, crucial to model our RS Loss, and (iii) results in a simple ``Identity Update'' rule (orange arrow in Step 2): $\Delta x_{ij}=L_{ij}$.
    \label{fig:RankBasedLosses}
} 
\end{figure}

\subsection{Revisiting the Incorporation of Error-Driven Optimization into Backpropagation}
\label{subsec:Errordriven}

\textbf{Definition of the Loss.} Oksuz et al. \cite{aLRPLoss} propose writing a ranking-based loss as $\mathcal{L}= \frac{1}{Z} \sum \limits_{i\in \mathcal{P}} \ell(i)$ where $Z$ is a problem specific normalization constant, $\mathcal{P}$ is the set of positive examples and $\ell(i)$ is the error term computed on $i \in \mathcal{P}$.

\textbf{Computation of the Loss.} Given logits ($s_i$), $\mathcal{L}$ can be computed in three steps \cite{APLoss,aLRPLoss} (Fig. \ref{fig:RankBasedLosses} green arrows):

{\noindent}\textit{Step 1}. The difference transform between logits $s_i$ and $s_j$ is computed by $x_{ij}=s_j-s_i$.

{\noindent}\textit{Step 2}. Using $x_{ij}$, errors originating from each pair of examples are calculated as primary terms ($L_{ij}$):
%
    \begin{align}
        \label{eq:GeneralPrimaryTermDefinition}
        L_{ij} = \begin{cases} \ell (i) p(j|i), & \mathrm{for}\;i \in \mathcal{P}, j \in \mathcal{N} \\
        0, & \mathrm{otherwise},
        \end{cases}
    \end{align}
where $p(j|i)$ is a probability mass function (pmf) that distributes $\ell (i)$, the error computed on $i \in \mathcal{P}$, over $j \in \mathcal{N}$ where $\mathcal{N}$ is the set of negative examples. By definition, the ranking-based error $\ell (i)$, and thus $L_{ij}$, requires pairwise-binary-ranking relation between outputs $i$ and $j$, which is determined by the non-differentiable unit step function $\mathrm{H}(x)$ (i.e. $\mathrm{H}(x)=1$ if $x \geq 0$ and $\mathrm{H}(x)=0$ otherwise) with input $x_{ij}$. 

Using $\mathrm{H}(x_{ij})$, different ranking-based functions can be introduced to define $\ell (i)$ and $p(j|i)$: e.g. the rank of the $i$th example, $\mathrm{rank}(i)=\sum \limits_{j \in \mathcal{P} \cup \mathcal{N}} \mathrm{H}(x_{ij})$; the rank of the $i$th example among positives, $\mathrm{rank^+}(i)= \sum \limits_{j \in \mathcal{P}} \mathrm{H}(x_{ij})$; and number of false positives with logits larger than $s_i$, $\mathrm{N_{FP}}(i)= \sum \limits_{j \in \mathcal{N}} \mathrm{H}(x_{ij})$. As an example, for AP Loss \cite{APLoss}, using these definitions, $\ell (i)$ and $p(j|i)$ can be simply defined as $\frac{\mathrm{N_{FP}}(i)}{\mathrm{rank}(i)}$ and $\frac{\mathrm{H}(x_{ij})}{\mathrm{N_{FP}}(i)}$ respectively \cite{aLRPLoss}.
    
{\noindent}\textit{Step 3}. Finally, $\mathcal{L}$ is calculated as the normalized sum of the primary terms \cite{aLRPLoss}: $\mathcal{L} =\frac{1}{Z} \sum \limits_{i\in \mathcal{P}} \ell(i)=\frac{1}{Z}\sum \limits_{i \in \mathcal{P} }\sum \limits_{j \in \mathcal{N} }  L_{ij}$.

\textbf{Optimization of the Loss.} Here, the aim is to find updates $\frac{\partial \mathcal{L}}{\partial s_i}$, and then proceed with backpropagation through model parameters. Among the three computation steps (Fig. \ref{fig:RankBasedLosses} orange arrows), Step 1 and Step 3 are differentiable, whereas a primary term $L_{ij}$ is not a differentiable function of difference transforms. Denoting this update in $x_{ij}$ by $\Delta x_{ij}$ and using the chain rule, $\frac{\partial \mathcal{L}}{\partial s_i}$ can be expressed as:
\small
\begin{align}
    \label{eq:Gradients}
    \frac{\partial \mathcal{L}}{\partial s_i} 
    = \sum \limits_{j,k} \frac{\partial \mathcal{L}}{\partial L_{jk}} \Delta x_{jk} \frac{\partial x_{jk}}{\partial s_i} 
    = \frac{1}{Z} \Big( \sum \limits_{j} \Delta x_{ji} - \sum \limits_{j} \Delta x_{ij} \Big). 
\end{align}
\normalsize
Chen et al. \cite{APLoss} incorporate the error-driven update \cite{Rosenblatt} and replace $\Delta x_{ij}$ by $-(L_{ij}^*-L_{ij})$ where $L_{ij}^*$ is the target primary term indicating the desired error for pair $(i, j)$. Both AP Loss \cite{APLoss} and aLRP Loss \cite{aLRPLoss} are optimized this way.%Using this method AP Loss \cite{APLoss} and aLRP Loss \cite{aLRPLoss} are shown to be optimized.

\subsection{Our Reformulation: Identity Update}
\label{subsec:IdentityUpdate}
We first identify two drawbacks of the formulation in Section \ref{subsec:Errordriven}: (D1) Resulting loss value ($\mathcal{L}$) does not consider the target $L_{ij}^*$, and thus, is not easily interpretable when $L_{ij}^* \neq 0$ (cf. aLRP Loss \cite{aLRPLoss} and our RS Loss - Section \ref{sec:RankSortLoss}); (D2) Eq. \ref{eq:GeneralPrimaryTermDefinition} assigns a non-zero primary term only if $i \in \mathcal{P}$ and $j \in \mathcal{N}$, effectively ignoring intra-class errors. These errors become especially important with continuous labels: The larger the label of $i \in \mathcal{P}$, the larger should $s_i$ be. %hence it is limited in addressing intra-class errors, which is crucial, e.g., when the labels are between $0$ and $1$, implying the larger $i \in \mathcal{P}$ has a label, the larger output $s_i$ is to be output by the model; else the ensuing error among positives is to be captured during training, which is not feasible following Eq. \ref{eq:GeneralPrimaryTermDefinition}.

\textbf{Definition of the Loss.} We  redefine the loss function as:
\begin{align}
\label{eq:LossIdentityUpdate}
\mathcal{L}= \frac{1}{Z}\sum \limits_{i \in \mathcal{P} \cup \mathcal{N}} (\ell(i) - \ell^*(i)),    
\end{align}
where $\ell^*(i)$ is the desired error term on $i \in \mathcal{P}$. Our loss definition has two benefits: (i) $\mathcal{L}$ directly measures the difference between the target and the desired errors, yielding an interpretable loss value to address (D1), and %second for the generalization purpose, 
(ii) we do not constrain $\mathcal{L}$ to be defined only on positives and replace ``$i \in \mathcal{P}$" with ``$i \in \mathcal{P} \cup \mathcal{N}$". Although we do not use ``$i \in \mathcal{P} \cup \mathcal{N}$" to model RS Loss, it makes the definition of $\mathcal{L}$ complete in the sense that, if necessary to obtain $\mathcal{L}$, individual errors ($\ell(i)$) can be computed on each output, and hence, $\mathcal{L}$ can be approximated more precisely or a larger set of ranking-based loss functions can be represented.

\textbf{Computation of the Loss.} In order to compute $\mathcal{L}$ (Eq. \ref{eq:LossIdentityUpdate}), we only replace Eq. \ref{eq:GeneralPrimaryTermDefinition} with:
\begin{align}
    \label{eq:PrimaryTermIdentityUpdate}
    L_{ij} = \left(\ell(i) - \ell^*(i) \right) p(j|i),
\end{align}
in three-step algorithm (Section \ref{subsec:Errordriven}, Fig. \ref{fig:RankBasedLosses} green arrows) and allow all pairs to have a non-zero error, addressing (D2).

\textbf{Optimization of the Loss.} Since the error of a pair, $L_{ij}$, is minimized when $\ell(i)=\ell^*(i)$, Eq. \ref{eq:PrimaryTermIdentityUpdate} has a target of $L^*_{ij}=0$ regardless of $\mathcal{L}$. Thus,  $\Delta x_{ij}$ in Eq. \ref{eq:Gradients} is simply the primary term itself: $\Delta x_{ij}=-(L^*_{ij}-L_{ij})=-(0-L_{ij})=L_{ij}$, concluding the derivation of our \textit{Identity Update}.


==> RankSort (arXiv)/sections/4.RankSortLoss.tex <==
\section{Rank \& Sort Loss}
\label{sec:RankSortLoss}
%Our Rank\&Sort (RS) Loss is different from the existing methods in that not only it is a purely ranking-based loss function, hence robust to class imbalance, but also it supervises object detectors and instance segmentation methods by using continuous localization qualities (e.g. IoU is between $0$ and $1$). Particularly, 
In order to supervise the classifier of visual detectors by considering the localisation qualities of the predictions (e.g. IoU), RS Loss decomposes the problem  into two tasks: (i) \textit{Ranking task}, which aims to rank each positive higher than all negatives, and (ii) \textit{sorting task}, which  aims to sort the logits $s_i$ in descending order wrt. continuous labels $y_i$ (e.g. IoUs). We define RS Loss and compute its gradients using our Identity Update (Section \ref{subsec:IdentityUpdate} -- Fig. \ref{fig:RankBasedLosses}).

\textbf{Definition.} Given logits $s_i$
%\footnote{Similar to previous work \cite{APLoss,aLRPLoss}, our formulation is based on logits instead of probabilities (i.e. scores obtained by applying sigmoid function to these logits). Note that since sigmoid is a strictly increasing function, the order will be preserved in both cases.} 
and their continuous labels $y_i \in [0,1]$ (e.g. IoU), we define RS Loss as the average of the differences between the current ($\ell_{\mathrm{RS}}(i)$) and target ($\ell_{\mathrm{RS}}^*(i)$) RS errors over positives (i.e. $y_i > 0$):
\begin{align}
\label{eq:RSLoss}
    \mathcal{L}_\mathrm{RS}:=\frac{1}{|\mathcal{P}|}\sum \limits_{i \in \mathcal{P}}  \left( \ell_{\mathrm{RS}}(i)-\ell_{\mathrm{RS}}^*(i) \right),
\end{align}
where $\ell_{\mathrm{RS}}(i)$ is a summation of the current ranking error and current sorting error:
%
\begin{align}
\label{eq:RSCurrent}
    \ell_{\mathrm{RS}}(i):= \underbrace{ \frac{\mathrm{N_{FP}}(i)}{\mathrm{rank}(i)}}_{\ell_{\mathrm{R}}(i):\ \text{Current Ranking Error}}
    +\underbrace{\frac{\sum \limits_{j \in \mathcal{P}} \mathrm{H}(x_{ij})(1-y_j)}{\mathrm{rank^+}(i)}}_{\ell_{\mathrm{S}}(i):\ \text{Current Sorting Error}}. 
\end{align}
%
For $i \in \mathcal{P}$, while the ``current ranking error'' is simply the precision error, the ``current sorting error''  penalizes the positives with  logits larger than $s_i$ by the average of their inverted labels, $1-y_j$. % of $j \in \mathcal{P}$ with larger logits as a measure to be compared against its target, which is defined based on the target ranking of $i \in \mathcal{P}$ (see target rankings in grey boxes for examples in Fig. \ref{fig:RSLoss}). 
Note that when $i \in \mathcal{P}$ is ranked above all $j \in \mathcal{N}$, $\mathrm{N_{FP}}(i)=0$ and target ranking error, $\ell^*_{\mathrm{R}}(i)$, is $0$. For target sorting error, we average over the inverted labels of $j \in \mathcal{P}$ with larger logits ($\mathrm{H}(x_{ij})$) and labels ($y_j \geq y_i$) than $i \in \mathcal{P}$ corresponding to the desired sorted order,
\begin{align}
\label{eq:RSTarget}
    \ell^*_{\mathrm{RS}}(i)= \cancelto{0}{\ell^*_{\mathrm{R}}(i)}+ \underbrace{\frac{\sum \limits_{j \in \mathcal{P}} \mathrm{H}(x_{ij})[y_j \geq y_i](1-y_j)}{\sum \limits_{j \in \mathcal{P}} \mathrm{H}(x_{ij})[y_j \geq y_i]}}_{\ell^*_{\mathrm{S}}(i):\text{Target Sorting Error}},
\end{align}
where $[\mathrm{P}]$ is the Iverson Bracket (i.e. 1 if predicate $\mathrm{P}$ is True; else 0), and similar to previous work \cite{APLoss}, $\mathrm{H}(x_{ij})$ is smoothed in the interval $[-\delta_{RS},\delta_{RS}]$ as $x_{ij} / 2 \delta_{RS}+0.5$.

\textbf{Computation.} We follow the three-step algorithm (Section \ref{sec:IdentityUpdate}, Fig. \ref{fig:RankBasedLosses}) and define primary terms, $L_{ij}$, using Eq. \ref{eq:PrimaryTermIdentityUpdate}, which allows us to express the errors among positives as:
    \begin{align}\footnotesize
        \label{eq:RSPrimaryTermDefinition}
        L_{ij} = \begin{cases} \left(\ell_{\mathrm{R}}(i) - \ell^*_{\mathrm{R}}(i) \right) p_{R}(j|i), & \mathrm{for}\; i \in \mathcal{P}, j \in \mathcal{N} \\
        \left(\ell_{\mathrm{S}}(i) - \ell^*_{\mathrm{S}}(i) \right) p_{S}(j|i), & \mathrm{for}\;i \in \mathcal{P}, j \in \mathcal{P},\\
        0, & \mathrm{otherwise},
        \end{cases}
    \end{align}
where ranking ($p_{R}(j|i)$) and sorting pmfs ($p_{S}(j|i)$) uniformly distribute ranking and sorting errors on $i$ respectively over examples causing error (i.e. for ranking, $j \in \mathcal{N}$ with $s_j>s_i$; for sorting, $j \in \mathcal{P}$ with $s_j>s_i$ but $y_j < y_i$): 
\begin{align}
    \label{eq:RSpmf}\footnotesize
        p_{R}(j|i) = \frac{\mathrm{H}(x_{ij})}{\sum \limits_{k \in \mathcal{N}}\mathrm{H}(x_{ik})}; p_{S}(j|i) = \frac{\mathrm{H}(x_{ij})[y_j < y_i]}{\sum \limits_{k \in \mathcal{P}} \mathrm{H}(x_{ik})[y_k < y_i]},
\end{align}

\textbf{Optimization.} To obtain $\frac{\partial \mathcal{L}_{\mathrm{RS}}}{\partial s_i}$, we simply replace $\Delta x_{ij}$ (Eq. \ref{eq:Gradients}) by the primary terms of RS Loss, $L_{ij}$ (Eq. \ref{eq:RSPrimaryTermDefinition}), following Identity Update (Section \ref{subsec:IdentityUpdate}). The resulting $\frac{\partial \mathcal{L}_{\mathrm{RS}}}{\partial s_i}$ for $i \in \mathcal{N}$ then becomes  (see Appendix \ref{sec:RSLossDetails} for derivations):
    \begin{align}
    \label{eq:RSNegGradients}
       \frac{\partial \mathcal{L}_{\mathrm{RS}}}{\partial s_i} = \frac{1}{|\mathcal{P}|}\sum \limits_{j \in \mathcal{P}} \ell_{\mathrm{R}}(j)p_{R}(i|j).
    \end{align}
Owing to the additional sorting error (Eq. \ref{eq:RSCurrent}, \ref{eq:RSTarget}), $\frac{\partial \mathcal{L}_{\mathrm{RS}}}{\partial s_i}$ for $i \in \mathcal{P}$ includes update signals for both promotion and demotion to sort the positives accordingly:
\begin{align}
    \label{eq:RSPosGradients}
    \frac{1}{|\mathcal{P}|} \Big( \underbrace{\ell^*_{\mathrm{RS}}(i)-\ell_{\mathrm{RS}}(i)}_{\text{Update signal to promote $i$}} +\underbrace{ \sum \limits_{j \in \mathcal{P} } \left( \ell_{\mathrm{S}}(j)- \ell^*_{\mathrm{S}}(j) \right)  p_{S}(i|j)} _{\text{Update signal to demote $i$}} \Big).
\end{align}
%
Note that the directions of the first and second part of Eq. \ref{eq:RSPosGradients} are different. To place $i\in \mathcal{P}$ in the desired ranking,  $\ell^*_{\mathrm{RS}}(i)-\ell_{\mathrm{RS}}(i) \leq 0$ promotes $i$ based on the error computed on itself, whereas $  \left( \ell_{\mathrm{S}}(j)- \ell^*_{\mathrm{S}}(j) \right) p_{S}(i|j) \geq 0$ demotes $i$ based on the signal from $j \in \mathcal{P}$. We provide more insight for RS Loss on an example in Appendix \ref{sec:RSLossDetails}.


==> RankSort (arXiv)/sections/5.RankSortforVisualDetection.tex <==
\section{Using RS Loss to Train Visual Detectors}

\begin{figure}
    \centerline{
        \includegraphics[width=0.45\textwidth]{figures/Architecture.pdf}
    }
    \caption{(a) A generic visual detection pipeline includes many heads from possibly multiple stages. An aux. head, in addition to the standard ones, is common in recent methods (e.g. centerness head for ATSS \cite{ATSS}, IoU head for IoU-Net \cite{IoUNet},  and mask IoU head for Mask-scoring R-CNN \cite{maskscoring}) to regress localisation quality and prioritize examples during inference (e.g. by multiplying classification scores by the predicted localisation quality). Sampling heuristics are also common to ensure balanced training. Such architectures use many hyper-parameters and are sensitive for tuning. (b) Training detectors with our RS Loss removes (i) aux. heads by directly supervising the classification (Cls.) head with continuous IoUs (in red \& bold), (ii) sampling heuristics owing to its robustness against class imbalance. We use losses with similar range with our RS Loss in other branches (i.e. GIoU Loss, Dice Loss) also by weighting each by using classification scores, obtained applying sigmoid to logits. (c) Instead of tuning $\lambda_{t}^k$s, we simply balance tasks by considering loss values. With this design, we train several detectors only by tuning the learning rate and improve their performance consistently. 
    \label{fig:Architecture}
} 
\end{figure}
\label{sec:SimpleBaseline}
This section develops an overall loss function to train detectors with RS Loss, in which only the learning rate needs tuning. As commonly performed in the literature \cite{GFL,paa}, Section \ref{subsec:Analysis} analyses different design choices on ATSS \cite{ATSS}, a SOTA one-stage object detector (i.e. $k=1$ in Eq. \ref{eq:LossVisualDetection}); and Section \ref{subsec:Extension} extends our design to other architectures.

\subsection{Dataset and Implementation Details}
Unless explicitly specified, we use (i) standard configuration of each detector and only replace the loss function, (ii) mmdetection framework \cite{mmdetection}, (iii) 16 images with a size of $1333 \times 800$ in a single batch ($4$ images/GPU, Tesla V100) during training, (iv) $1\times$ training schedule (12 epochs),  (v) single-scale test with images with a size of $1333 \times 800$, (vi) ResNet-50 backbone with FPN \cite{FeaturePyramidNetwork}, (vii) COCO \textit{trainval35K} (115K images) and \textit{minival} (5k images) sets \cite{COCO} to train and test our models, (iix) report COCO-style AP.

\subsection{Analysis and Tuning-Free Design Choices}
\label{subsec:Analysis}
ATSS \cite{ATSS} with its classification, box regression and centerness heads is originally trained by minimizing:
\begin{align}
    \label{eq:LossATSS}
    \mathcal{L}_{ATSS}=\mathcal{L}_{cls}+ \lambda_{box} \mathcal{L}_{box} + \lambda_{ctr} \mathcal{L}_{ctr},
\end{align}
where $\mathcal{L}_{cls}$ is Focal Loss \cite{FocalLoss}; $\mathcal{L}_{box}$ is GIoU Loss \cite{GIoULoss}; $\mathcal{L}_{ctr}$ is Cross-entropy Loss with continuous labels to supervise  centerness prediction; and $\lambda_{box}=2$ and $\lambda_{ctr}=1$. We first remove the centerness head and replace $\mathcal{L}_{cls}$ by our RS Loss (Section \ref{sec:RankSortLoss}), $\mathcal{L}_{RS}$, using $\mathrm{IoU}(\hat{b}_i, b_i)$ between a prediction box ($\hat{b}_i$) and ground truth box ($b_i$) as the continuous labels:
\begin{align}
    \label{eq:LossATSSRS}
    \mathcal{L}_{RS-ATSS}=\mathcal{L}_{RS}+ \lambda_{box} \mathcal{L}_{box},
\end{align}
where $\lambda_{box}$, the \textit{task-level balancing coefficient}, is generally set to a constant scalar by grid search. 

Inspired by recent work \cite{aLRPLoss,SamplingHeuristics}, we investigate two tuning-free heuristics to determine  $\lambda_{box}$ every iteration: (i) value-based: $\lambda_{box} = \mathcal{L}_{RS}/\mathcal{L}_{box}$, and (ii) magnitude-based: $\lambda_{box}= \abs{ \frac{{\partial \mathcal{L}}_{\mathrm{RS}}}{{\partial \mathbf{\hat{s}}}}} / \abs{ \frac{{\partial \mathcal{L}}_{\mathrm{box}}}{{\partial \mathbf{b}}}}$ where $\abs{\cdot}$ is L1 norm, $\mathbf{\hat{b}}$ and $\mathbf{s}$ are box regression and classification head outputs respectively. In our analysis on ATSS trained with RS Loss, we observed that value-based task balancing performs similar to tuning $\lambda_{box}$ ($\smallsim 0$ AP difference on average). Also, we use score-based weighting \cite{GFL} by multiplying the GIoU Loss of each prediction using its classification score (details are in Appendix \ref{sec:Analysis}). Note that value-based task balancing and score-based instance weighting are both hyper-parameter-free and easily applicable to all networks. \textit{With these design choices, Eq. \ref{eq:LossATSSRS} has only $1$ hyper-parameter} (i.e. $\delta_{RS}$ in $\mathrm{H}(\cdot)$, set to $0.50$, to smooth the unit-step function)

\subsection{Training Different Architectures}
\label{subsec:Extension}
Fig. \ref{fig:Architecture} presents a comparative overview on how we adopt RS Loss to train different architectures: When we use RS Loss to train the classifier (Fig. \ref{fig:Architecture}(b)), we remove aux. heads (e.g. IoU head in IoU-Net \cite{IoUNet}) and sampling heuristics (e.g. OHEM in YOLACT \cite{yolact}, random sampling in Faster R-CNN \cite{FasterRCNN}). We adopt score-based weighting in box regression and mask prediction heads, and prefer Dice Loss, instead of the common Cross-entropy Loss, to train mask prediction head for instance segmentation due to (i) its bounded range (between $0$ and $1$), and (ii) holistic evaluation of the predictions, both similar to GIoU Loss. Finally, we set $\lambda_{t}^k$ (Eq. \ref{eq:LossVisualDetection}) to scalar $\mathcal{L}_{cls}^k/\mathcal{L}_{t}^k$ (i.e. $\mathcal{L}_{cls} = \mathcal{L}_{RS}$) every iteration (Fig. \ref{fig:Architecture}(c)) with the single exception of RPN where we multiply the losses of RPN by $0.20$ following aLRP Loss. 





==> RankSort (arXiv)/sections/6.Experiments.tex <==
\section{Experiments}
\label{sec:Experiments}
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.16em}
    \footnotesize
    \caption{RS-R-CNN uses the standard IoU-based assigner, is sampling-free, employs no aux. head, is almost tuning-free wrt. task-balancing weights ($\lambda_{t}^k$s -- Eq. \ref{eq:LossVisualDetection}), and thus, has the least number of hyper-parameters (H\# = $3$ -- two $\delta_{RS}$, one for each RS Loss to train RPN \& R-CNN, and one RPN weight). Still, RS-R-CNN improves standard Faster R-CNN with FPN by $\smallsim3$ AP; aLRP Loss (ranking-based loss baseline) by $\smallsim2$ AP; IoU-Net (a method with IoU head) by $1.5$ AP. RS-R-CNN+ replaces upsampling of FPN by lightweight Carafe operation \cite{carafe} and maintains $\smallsim2$ AP gap from Carafe FPN ($38.6$ to $40.8$ AP). All models use ResNet-50, are evaluated in COCO \textit{minival} and trained for 12 epochs on mmdetection except for IoU-Net. 
    %and KL Loss. Var.: Variance. 
    H\#: Number of hyper-parameters (Appendix \ref{sec:Experiments_supp} presents details on H\#.)}
    \label{tab:TwoStage}
    \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|c||c||c|} \hline
    Method&Assigner&Sampler&Aux. Head&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$&$ \mathrm{oLRP_{Loc}} \downarrow$&$ \mathrm{oLRP_{FP}} \downarrow$&$ \mathrm{oLRP_{FN}} \downarrow$&H\# $\downarrow$&Venue\\ \hline
    FPN \cite{FeaturePyramidNetwork}& IoU-based&Random&None&$36.5$&$58.5$&$39.4$&$70.1$&$18.3$&$27.8$&$45.8$&$9$&CVPR 17\\
    %OHEM \cite{OHEM}& IoU-based &OHEM& & & & & & & & & CVPR 16\\
    %L1 Loss \cite{mmdetection}& IoU-based&Random&$37.4$&$58.1$&$40.4$&$69.6$&$17.5$&$27.9$&$46.4$& -- (?)\\
    aLRP Loss \cite{aLRPLoss}& IoU-based&None&None&$37.4$&$57.9$&$39.2$&$69.2$&$17.6$&$28.5$&$46.1$ &$\mathbf{3}$&NeurIPS 20\\
    GIoU Loss \cite{GIoULoss}& IoU-based&Random&None&$37.6$&$58.2$&$41.0$&$69.2$&$17.0$&$28.5$&$46.3$&$7$&CVPR 19\\
    %Sparse R-CNN \cite{sparsercnn}&Hungarian&None&$37.9$&$56.0$&$40.5$&$69.2$&$15.8$&$28.6$&$48.5$&CVPR 21\\
    IoU-Net \cite{IoUNet}& IoU-based&Random&IoU Head&$38.1$&$56.3$&--&--&--&--&--&$11$&ECCV 18\\
    Libra R-CNN \cite{LibraRCNN}& IoU-based&IoU-based&None&$38.3$&$59.5$&$41.9$&$68.8$&$17.2$&$27.5$&$45.4$&$11$&CVPR 19\\
    AutoLoss-A \cite{autoloss}& IoU-based&Random&None&$38.5$&$58.6$&$41.8$&$68.4$&$16.6$&$27.1$&$45.5$&$7$&ICLR 21\\
    Carafe FPN \cite{carafe}&IoU-based&Random&None&$38.6$&$59.9$&$42.2$&$68.3$&$17.2$&$27.0$&$44.2$&$7$&ICCV 19\\  
    % KL Loss \cite{KLLoss}& IoU-based&Random&Var. Head&$38.8$&$57.8$&$41.6$&--&--&--&--&$10$&CVPR 19\\
    Dynamic R-CNN \cite{dynamicrcnn}&Dynamic&Random&None&$38.9$&$57.6$&$42.7$&$68.2$&$\mathbf{15.7}$&$27.7$&$46.6$&$10$&ECCV 20\\ \hline 
    RS-R-CNN (Ours)&IoU-based&None&None&$39.6$&$59.5$&$43.0$&$67.9$&$16.3$&$27.8$&$45.4$&$\mathbf{3}$&\\ 
    RS-R-CNN+ (Ours)&IoU-based&None&None&$\mathbf{40.8}$&$\mathbf{61.4}$&$\mathbf{43.8}$&$\mathbf{66.9}$&$16.3$&$\mathbf{26.4}$&$\mathbf{43.7}$&$\mathbf{3}$&\\ \hline 
    \end{tabular}
\end{table*}

To present the contribution of RS Loss in terms of performance and tuning simplicity, we conduct experiments on seven visual detectors with a diverse set of architectures: four object detectors (i.e. Faster R-CNN \cite{FasterRCNN}, Cascade R-CNN \cite{CascadeRCNN}, ATSS \cite{ATSS} and PAA \cite{paa} -- Section \ref{subsec:ObjectDetection}) and three instance segmentation methods (i.e. Mask R-CNN \cite{MaskRCNN}, YOLACT \cite{yolact} and SOLOv2 \cite{solov2} -- Section \ref{subsec:InstanceSegm}). Finally, Section \ref{subsec:Ablation} presents ablation analysis.
%and one keypoint detector (i.e. Keypoint R-CNN \cite{MaskRCNN} -- Section \ref{subsec:KeypointDet}).  

\subsection{Experiments on Object Detection}
\label{subsec:ObjectDetection}
% We train multi- and one-stage detectors with RS Loss.

\subsubsection{Multi-stage Object Detectors}
\label{subsubsec:multistage}
To train Faster R-CNN \cite{FasterRCNN} and Cascade R-CNN \cite{CascadeRCNN} by our RS Loss (i.e. RS-R-CNN), we remove sampling from all stages (i.e. RPN and R-CNNs), use all anchors to train RPN and $m$ top-scoring proposals/image (by default, $m=1000$ for Faster R-CNN and $m=2000$ Cascade R-CNN in mmdetection \cite{mmdetection}), replace softmax classifiers by binary sigmoid classifiers and set the initial learning rate to $0.012$.

%\textbf{Comparison with different R-CNN variants:}
RS Loss reaches $39.6$ AP on a standard Faster R-CNN and outperforms (Table \ref{tab:TwoStage}): (i) FPN \cite{FeaturePyramidNetwork} (Cross-entropy \& Smooth L1 losses) by $3.4$ AP, (ii) aLRP Loss \cite{aLRPLoss}, a SOTA ranking-based baseline, by $2.2$ AP, (iii) IoU-Net \cite{IoUNet} with aux. head by $1.5$ AP and (iv) Dynamic R-CNN, closest counterpart, by $0.7$ AP. We, then, use the lightweight Carafe \cite{carafe} as the  upsampling operation in FPN and obtain $40.8$ AP (RS-R-CNN+), still maintaining $\smallsim2$ AP gap from Carafe FPN \cite{carafe} ($38.6$ AP) and outperforming all methods in all AP- and oLRP-based \cite{LRP,LRParXiv} performance measures except $\mathrm{oLRP_{Loc}}$, which implies that our main contribution is in classification task trained by our RS Loss and there is still room for improvement in the localisation task. RS Loss also improves the stronger baseline Cascade R-CNN \cite{CascadeRCNN} by $1$ AP from $40.3$ AP to $41.3$ AP (Appendix \ref{sec:Experiments_supp} presents detailed results for Cascade R-CNN). %\textbf{Simplification of training:} 
Finally, RS Loss has the least number of hyper-parameters (H\# = $3$, Table \ref{tab:TwoStage}) and does not need  a sampler, an aux. head  or  tuning of $\lambda_{t}^k$s (Eq. \ref{eq:LossVisualDetection}).


\comment{
\begin{table}
    \centering
    \footnotesize
    \caption{\textbf{Improvements to obtain RSVD R-CNN+}}
    \label{tab:Improvements}
    \begin{tabular}{|c|c|c|c||c|c|c|} \hline
    Dyn.Ass.&Carafe&Head+&Cos.Ann.&AP&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$\\ \hline 
     & & & &$39.6$&$59.5$&$43.0$ \\ \hline
    \checkmark& & & &$39.4$&$59.5$&$42.6$\\
    &\checkmark&& &$40.8$&$61.4$&$43.8$\\
    & &\checkmark & &$39.6$&$58.6$&$43.0$\\
    & & &\checkmark &$39.3$ &$59.6$&$42.5$\\  \hline
    \checkmark &\checkmark &\checkmark &\checkmark& & &\\  \hline
    \end{tabular}
\end{table}
}


\subsubsection{One-stage Object Detectors}

\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.5em}
    \footnotesize
    \caption{RS Loss has the least number of hyper-parameters (H\#) and outperforms (i) rank-based alternatives significantly, (ii) the default setting with an aux. head (underlined) by $0.6$ AP, (iii) score-based alternative, QFL, especially on PAA. We test unified losses (i.e. a loss considering localisation quality while training classification head) only without aux. head. All models use ResNet-50.}
    \label{tab:OneStage}
    \begin{tabular}{|c|c|c|c||c|c|c||c||c|c|c|c||c|} \hline
    \multirow{2}{*}{Loss Function}&\multirow{2}{*}{Unified}&\multirow{2}{*}{Rank-based}&\multirow{2}{*}{Aux. Head}& \multicolumn{4}{|c|}{ATSS \cite{ATSS}}&\multicolumn{4}{|c|}{PAA \cite{paa}}&\multirow{2}{*}{H\# $\downarrow$}\\ \cline{5-12}
    & & & &AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$ &\\ \hline
    \multirow{2}{*}{Focal Loss \cite{FocalLoss}}& & & &$38.7$&$57.6$&$41.5$&$68.9$ &$39.9$&$57.3$&$43.4$&$68.7$&$3$\\
    & & &\checkmark&\underline{$39.3$}&\underline{$57.5$}&\underline{$42.6$}&\underline{$68.6$} &\underline{$40.4$}&\underline{$58.4$}&\underline{$43.9$}&\underline{$67.7$}&\underline{$4$}\\ \hline
    \multirow{2}{*}{AP Loss \cite{APLoss}}& &\checkmark& &$38.1$&$58.2$&$41.0$&$69.2$ &$35.3$&$53.1$&$38.5$&$71.5$&$2$\\
    & &\checkmark&\checkmark&$37.2$&$55.6$&$40.2$&$70.0$&$37.3$&$54.3$&$41.2$&$70.5$&$3$\\ \hline
    QFL \cite{GFL} &\checkmark& & &$39.7$&$58.1$&$\mathbf{42.7}$&$68.0$&$40.2$&$57.4$&$43.8$&$68.3$&$2$\\ \hline
    aLRP Loss \cite{aLRPLoss}&\checkmark&\checkmark& &$37.7$&$57.4$&$39.9$&$69.4$ &$37.7$&$56.1$&$40.1$&$69.9$&$\mathbf{1}$\\ \hline
    RS Loss (Ours) &\checkmark&\checkmark& &$\mathbf{39.9}$&$\mathbf{58.9}$&$42.6$&$\textbf{67.9}$&$\mathbf{41.0}$&$\mathbf{59.1}$&$\mathbf{44.5}$&$\textbf{67.3}$&$\mathbf{1}$\\ \hline
    \end{tabular}
\end{table*}
We train ATSS \cite{ATSS} and PAA \cite{paa} including a centerness head and an IoU head respectively in their architectures. We adopt the anchor configuration of Oksuz et al. \cite{aLRPLoss} for all ranking-based losses (different anchor configurations do not affect performance of standard ATSS \cite{ATSS}) and set learning rate to $0.008$. While training PAA, we keep the scoring function, splitting positives and negatives, for a fair comparison among different loss functions.

\textbf{Comparison with AP and aLRP Losses, ranking-based baselines:} We simply replaced Focal Loss by AP Loss to train networks, and as for aLRP Loss, similar to our RS Loss, we tuned its learning rate as $0.005$ due to its tuning simplicity. Both for ATSS and PAA, RS Loss provides significant gains over ranking-based alternatives, which were trained for 100 epochs using SSD-like augmentation \cite{SSD} in previous work \cite{APLoss,aLRPLoss}: $1.8$/$2.2$ AP gain for ATSS and $3.7$/$3.3$ gain for PAA for AP/aLRP Loss (Table \ref{tab:OneStage}).
 
\textbf{Comparison with Focal Loss, default loss function:} RS Loss provides around $\smallsim 1$ AP gain when both networks are equally trained without an aux. head (Table \ref{tab:OneStage}) and $0.6$ AP gain compared to the default networks with aux. heads.

\textbf{Comparison with QFL, score-based loss function using continuous IoUs as labels:} To apply QFL \cite{GFL} to PAA,  we remove the aux. IoU head (as we did with ATSS), test two possible options ((i) default PAA setting with $\lambda_{box}=1.3$ and IoU-based weighting, (ii) default QFL setting: $\lambda_{box}=2.0$ and score-based weighting) and report the best result for QFL. While the results of QFL and RS Loss are similar for ATSS, there is $0.8$ AP gap in favor of our RS Loss, which can be due to the different positive-negative assignment method of PAA (Table \ref{tab:OneStage}). 

\subsubsection{Comparison with SOTA}
Here, we use our RS-R-CNN since it yields the largest improvement over its baseline. %for which our performance improvement is more significant against baseline.
We train RS-R-CNN for 36 epochs using multiscale training by randomly resizing the shorter size within $[480, 960]$ on ResNet-101 with DCNv2 \cite{DCNv2}. Table \ref{tab:Detectiontestdev} reports the results on COCO \textit{test-dev}: Our RS-R-CNN reaches $47.8$ AP and outperforms similarly trained Faster R-CNN and Dynamic R-CNN by $\smallsim 3$ and $\smallsim 1$ AP respectively. Although we do not increase the number of parameters for Faster R-CNN, RS R-CNN outperforms all multi-stage detectors including TridentNet \cite{TridentNet}, which has more parameters. Our RS-R-CNN+ (Section \ref{subsubsec:multistage}) reaches $48.2$ AP, and RS-Mask R-CNN+ (Section \ref{subsec:InstanceSegm}) reaches $49.0$ AP, outperforming all one- and multi-stage counterparts.

\begin{table}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
    \caption{Comparison with SOTA for object detection on COCO \textit{test-dev} using ResNet-101 (except *) with DCN. The result of the similarly trained Faster R-CNN is acquired from Zhang et al. \cite{dynamicrcnn}.  +: upsampling of FPN is Carafe \cite{carafe}, *:ResNeXt-64x4d-101}
    \label{tab:Detectiontestdev}
    \begin{tabular}{|m{0.8em}|c||c|c|c|c|c|c|} \hline
    &Method&AP&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&$\mathrm{AP_{S}}$&$\mathrm{AP_{M}}$&$\mathrm{AP_{L}}$\\ \hline 
    \multirow{4}{*}{\rotatebox{90}{One-stage}}&ATSS \cite{ATSS}&$46.3$&$64.7$&$50.4$&$27.7$&$49.8$&$58.4$\\
    &GFL \cite{GFL}&$47.3$&$66.3$&$51.4$&$28.0$&$51.1$&$59.2$\\
    &PAA \cite{paa}&$47.4$&$65.7$&$51.6$&$27.9$&$51.3$&$60.6$\\
    &RepPointsv2 \cite{reppointsv2}&$48.1$&$67.5$&$51.8$&$28.7$&$50.9$&$60.8$\\ 
    % &GFLv2 \cite{GFLv2}&$48.3$&$66.5$&$52.8$&$28.8$&$51.9$&$60.7$\\ 
    \hline
    \multirow{4}{*}{\rotatebox{90}{Multi-stage}}&Faster R-CNN \cite{dynamicrcnn}&$44.8$&$65.5$&$48.8$&$26.2$&$47.6$&$58.1$\\
    &Trident Net \cite{TridentNet}&$46.8$&$67.6$&$51.5$&$28.0$&$51.2$&$60.5$ \\
    &Dynamic R-CNN \cite{dynamicrcnn}&$46.9$&$65.9$&$51.3$&$28.1$&$49.6$&$60.0$ \\
    &D2Det \cite{D2Det}&$47.4$&$65.9$&$51.7$&$27.2$&$50.4$&$61.3$\\ \hline
    \multirow{4}{*}{\rotatebox{90}{Ours}}&RS-R-CNN &$47.8$&$68.0$&$51.8$&$28.5$&$51.1$&$61.6$\\ 
    &RS-R-CNN+&$48.2$&$68.6$&$52.4$&$29.0$&$51.3$&$61.7$\\  
    &RS-Mask R-CNN+&$\mathbf{49.0}$&$\mathbf{69.2}$&$\mathbf{53.4}$&$\mathbf{29.9}$&$\mathbf{52.4}$&$\mathbf{62.8}$\\ \cline{2-8}
    &RS-Mask R-CNN+*&$50.2$&$70.3$&$54.8$&$31.5$&$53.5$&$63.9$\\ 
    %\cline{2-8} &RS-Mask R-CNN+$^*$&$50.4$&$70.6$&$55.1$&$32.9$&$53.8$&$62.0$\\  
    \hline
    \end{tabular}
\end{table}

\subsection{Experiments on Instance Segmentation}
\label{subsec:InstanceSegm}
%Similar to Section \ref{subsec:ObjectDetection}, we train multi- and one-stage methods with RS Loss and compare our results with SOTA.
%We train multi- and one-stage methods with RS Loss.

\subsubsection{Multi-stage Instance Segmentation Methods}
We train Mask R-CNN \cite{MaskRCNN} on COCO and LVIS datasets by keeping all design choices of Faster R-CNN the same.

\textbf{COCO:} We observe $\smallsim2$ AP gain for both segmentation and detection performance (Table \ref{tab:MaskRCNN}) over Mask R-CNN. Also, RS-Mask R-CNN outperforms Mask-scoring R-CNN \cite{maskscoring}, with an additional aux. mask IoU head, by $0.4$ mask AP, $1.8$ box AP and $0.9$ mask oLRP (Table \ref{tab:MaskRCNN}). 
%Compared to Mask R-CNN, one training iteration of RS-Mask R-CNN takes around $1.5 \times$ longer on average while RS Loss has no effect on inference time. %Similar to RS-R-CNN+, replacing the upsampling operation in FPN  by Carafe \cite{carafe} to obtain RS-Mask R-CNN+, boosts the performance to $37.3$ mask AP and $41.1$ box AP. 
\comment{
\begin{table*}
    \centering
    \footnotesize
    \caption{Without an aux. head, RS-Mask R-CNN improves Mask R-CNN by $\smallsim2$ AP and outperforms Mask-scoring R-CNN.}
    \label{tab:MaskRCNN}
    \begin{tabular}{|c|c||c|c|c|c||c|c|c|c||c|} \hline
    \multirow{2}{*}{Method}&\multirow{2}{*}{Aux. Head}& \multicolumn{4}{|c||}{Segmentation Performance}&\multicolumn{4}{|c|}{Detection Performance}&\multirow{2}{*}{H\# $\downarrow$}\\ \cline{3-10}
    & &AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$&\\ \hline
    Mask R-CNN \cite{MaskRCNN}&None&$34.7$&$55.7$&$37.2$&$71.2$&$38.2$&$58.8$&$41.4$&$68.7$&$8$\\ 
%    Cascade Mask R-CNN \cite{MaskRCNN}&$35.9$&$56.6$&$38.4$& &$41.2$&$59.4$&$45.0$& \\ 
    Mask-scoring R-CNN \cite{maskscoring}&mask IoU Head&$36.0$&$55.8$&$38.7$& $71.0$&$38.2$&$58.8$&$41.7$&$69.0$&$9$ \\ \hline
    RS-Mask R-CNN&None&$\mathbf{36.4}$&$\mathbf{57.3}$&$\mathbf{39.2}$&$\mathbf{70.1}$ &$\mathbf{40.0}$&$\mathbf{59.8}$&$\mathbf{43.4}$&$\mathbf{67.5}$&$\mathbf{3}$ \\  \hline
%    RS Cascade Mask R-CNN &$?$&$?$&$?$& &$?$&$?$&$?$& \\  
%    RS-Mask R-CNN +&$37.3$&$58.6$&$40.2$&$69.4$&$41.1$&$61.4$&$44.9$&$66.6$ \\ \hline
%    RS Cascade Mask R-CNN+&$?$&$?$&$?$& &$?$&$?$&$?$& \\ \hline
    \end{tabular}
\end{table*}
}
\begin{table}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.1em}
    \caption{Without an aux. head, RS-Mask R-CNN improves Mask R-CNN  \cite{MaskRCNN} by $\smallsim2$ AP and outperforms Mask-scoring R-CNN \cite{maskscoring} which employs an additional mask IoU head as aux. head.}
    \label{tab:MaskRCNN}
    \begin{tabular}{|c|c||c|c|c|c||c||c|} \hline
    \multirow{2}{*}{Method}&Aux& \multicolumn{4}{|c||}{Segmentation Performance}&\multirow{2}{*}{$\mathrm{AP_{box}}$}&\multirow{2}{*}{H\# $\downarrow$}\\ \cline{3-6}
    &Head&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$& &\\ \hline
    Mask R-CNN& &$34.7$&$55.7$&$37.2$&$71.2$&$38.2$&$8$\\ 
%    Cascade Mask R-CNN \cite{MaskRCNN}&$35.9$&$56.6$&$38.4$& &$41.2$&$59.4$&$45.0$& \\ 
    Mask-sc. R-CNN &\checkmark&$36.0$&$55.8$&$38.7$& $71.0$&$38.2$&$9$ \\ \hline
    RS-Mask R-CNN& &$\mathbf{36.4}$&$\mathbf{57.3}$&$\mathbf{39.2}$&$\mathbf{70.1}$ &$\mathbf{40.0}$&$\mathbf{3}$ \\  \hline
%    RS Cascade Mask R-CNN &$?$&$?$&$?$& &$?$&$?$&$?$& \\  
%    RS-Mask R-CNN +&$37.3$&$58.6$&$40.2$&$69.4$&$41.1$&$61.4$&$44.9$&$66.6$ \\ \hline
%    RS Cascade Mask R-CNN+&$?$&$?$&$?$& &$?$&$?$&$?$& \\ \hline
    \end{tabular}
\end{table}

\textbf{LVIS:} Replacing the Cross-entropy to train Mask R-CNN with repeat factor sampling (RFS) by our RS Loss improves the performance by $3.5$ mask AP on the long-tailed LVIS dataset ($21.7$ to $25.2$ with $\smallsim 7 \mathrm{AP_{r}}$ improvement on rare classes) and outperforms recent counterparts (Table \ref{tbl:LVIS}). 

\begin{table}
\setlength{\tabcolsep}{0.25em}
\footnotesize
\caption{Comparison on LVIS v1.0 val set. Models are trained with ResNet-50, multiscale images (range: $[640,800]$) for 12 epochs. 
%In addition, BAGS is finetuned for 12 epochs. 
\label{tbl:LVIS}} 
 \centering
\begin{tabular}{|c||c|c|c|c||c||c|}
\hline
Method&$\mathrm{AP_{mask}}$&$\mathrm{AP_{r}}$&$\mathrm{AP_{c}}$&$\mathrm{AP_{f}}$&$\mathrm{AP_{box}}$&Venue\\ \hline
RFS \cite{LVIS} &$21.7$&$9.6$&$21.0$&$27.8$&$22.5$&CVPR 19\\
BAGS \cite{BAGS}&$23.1$&$13.1$&$22.5$&$28.2$&$23.7$&CVPR 20 \\ 
Eq. Lossv2 \cite{Eqv2}&$23.7$&$14.9$&$22.8$&$28.6$&$24.2$&CVPR 21\\ \hline
RFS+RS Loss&$\mathbf{25.2}$&$\mathbf{16.8}$&$\mathbf{24.3}$&$\mathbf{29.9}$&$\mathbf{25.9}$& \\ \hline
\end{tabular}
\end{table}

\subsubsection{One-stage Instance Segmentation Methods}
Here, we train two different approaches with our RS Loss: (i) YOLACT \cite{yolact},  a real-time instance segmentation method, involving sampling heuristics (e.g. OHEM \cite{OHEM}), aux. head and carefully-tuned loss weights, and demonstrate RS Loss can discard all by improving its performance (ii) SOLOv2 \cite{solov2} as an anchor-free SOTA method.

\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
    \caption{RS-YOLACT does not employ any additional training heuristics and outperforms  YOLACT by significant margin.}
    \label{tab:Yolact}
    \begin{tabular}{|c|c|c|c||c|c|c||c||c|c|c|c||c|} \hline
    \multirow{2}{*}{Method}& \multicolumn{3}{|c||}{Additional Training Heuristics}& \multicolumn{4}{|c||}{Segmentation Performance}&\multicolumn{4}{|c|}{Detection Performance}&\multirow{2}{*}{H\# $\downarrow$}\\ \cline{2-12}
    &OHEM \cite{OHEM}&Size-based Norm.&Sem.Segm. Head&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$&oLRP $\downarrow$& \\ \hline
    \multirow{4}{*}{YOLACT \cite{yolact}}& \checkmark &\checkmark & \checkmark&$28.4$&$47.7$&$29.1$&$75.4$&$30.5$&$52.3$&$31.8$&$73.9$&$5$ \\
    & &\checkmark&\checkmark&$15.1$&$27.1$&$15.0$&$86.6$&$12.6$&$27.8$&$10.0$&$88.5$&$4$ \\
    &\checkmark& &\checkmark&$21.7$&$40.2$&$20.7$&$80.5$&$30.4$&$52.2$&$31.4$&$74.1$&$5$ \\
    &\checkmark&\checkmark& &$28.1$&$47.5$&$28.7$&$75.6$&$30.5$&$51.9$&$32.0$&$74.0$&$4$ \\
    & & & &$13.6$&$26.4$&$12.4$&$87.5$&$15.1$&$32.9$&$12.1$&$86.3$&$3$ \\ \hline
    %aLRP Loss& & & &$28.6$&$48.6$&$29.0$&$75.2$&$31.9$&$52.8$&$32.4$&$72.9$ \\ \hline
    RS-YOLACT& & & &$\mathbf{29.9}$&$\mathbf{50.5}$&$\mathbf{30.6}$& $\mathbf{74.7}$&$\mathbf{33.8}$&$\mathbf{54.2}$&$\mathbf{35.4}$&$\mathbf{71.8}$&$\mathbf{1}$ \\ \hline
    \end{tabular}
\end{table*}

\textbf{YOLACT:} Following YOLACT \cite{yolact}, we train and test RS-YOLACT by images with size $550 \times 550$ for $55$ epochs. Instead of searching for epochs to decay learning rate, carefully tuned for YOLACT as $20$, $42$, $49$ and $52$, we simply adopt cosine annealing with an initial learning rate of $0.006$. Then, we remove (i) OHEM, (ii) semantic segmentation head, (iii) carefully tuned task weights (i.e. $\lambda_{box}=1.5$, $\lambda_{mask}=6.125$) and (iv) size-based normalization (i.e. normalization of mask head loss of each instance by the ground-truth area). Removing each heuristic ensues a slight to significant performance drop (at least requires retuning of $\lambda_{t}$ -- Table \ref{tab:Yolact}). After these simplifications, our RS-YOLACT improves baseline by $1.5$ mask AP and $3.3$ box AP.
%, and (ii) ranking-based baseline, aLRP Loss, by $1.3$ mask AP and $1.9$ box AP.

\textbf{SOLOv2:} Following Wang et al. \cite{solov2}, we train anchor-free SOLOv2 with RS Loss for 36 epochs using multiscale training on its two different settings: (i) SOLOv2-light is the real-time setting with ResNet-34 and images with size $448 \times 448$ at inference. We use 32 images/batch and learning rate $0.012$ for training. (ii)  SOLOv2 is the SOTA setting with ResNet-101 and images with size $1333 \times 800$ at inference. We use 16 images/batch and learning rate $0.006$ for training. Since SOLOv2 does not have a box regression head, we use Dice coefficient as the continuous labels of RS Loss (see Appendix \ref{sec:Experiments_supp} for an analysis of using different localisation qualities as labels). Again, RS Loss performs better than the baseline (i.e. Focal Loss and Dice Loss) only by tuning the learning rate (Table \ref{tab:SOLOv2}).

\subsubsection{Comparison with SOTA}
We use our RS-Mask R-CNN (i.e. standard Mask R-CNN with RS Loss) to compare with SOTA methods. In order to fit in 16GB memory of our V100 GPUs and keep all settings unchanged, we limit the number of maximum proposals in the mask head by 200, which can simply be omitted for GPUs with larger memory. Following our counterparts \cite{solov2,centermask}, we first train RS-Mask R-CNN for 36 epochs with multiscale training between $[640,800]$ using ResNet-101 and reach $40.6$ mask AP (Table \ref{tab:Segmentationtestdev}), improving Mask R-CNN by $2.3$ mask AP and outperforming all SOTA methods by a notable margin ($\smallsim 1$ AP). Then, we train RS-Mask R-CNN+ (i.e. standard Mask R-CNN except upsampling of FPN is lightweight Carafe \cite{carafe}) also by extending the multiscale range to $[480,960]$ and reach $42.0$ mask AP, which even outperforms all models with DCN. With DCN \cite{DCNv2} on ResNet-101, our RS-Mask R-CNN+ reaches $43.9$ mask AP.

\begin{table}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.2em}
    \caption{Comparison on anchor-free SOLOv2.}
    \label{tab:SOLOv2}
    \begin{tabular}{|c|c||c|c|c||c||c|} \hline
    Method&Backbone&AP&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&oLRP $\downarrow$&H\# $\downarrow$ \\ \hline 
    SOLOv2-light&ResNet-34&$32.0$&$50.7$&$33.7$&$73.5$&$3$\\ 
    RS-SOLOv2-light&ResNet-34&$\mathbf{32.6}$&$\mathbf{51.7}$&$\mathbf{34.2}$&$\mathbf{72.7}$&$\mathbf{1}$\\ \hline
    SOLOv2&ResNet-101&$39.1$&$59.8$&$41.9$&$67.3$&$3$\\ 
    RS-SOLOv2&ResNet-101&$\mathbf{39.7}$&$\mathbf{60.6}$&$\mathbf{42.2}$&$\mathbf{66.9}$&$\mathbf{1}$\\ \hline
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.15em}
    \caption{Comparison with SOTA for instance segmentation on COCO \textit{test-dev}. All methods (except *) use ResNet-101. The result of the similarly trained Mask R-CNN is acquired from Chen et al. \cite{tensormask}. +: upsampling of FPN is Carafe, *:ResNeXt-64x4d-101}
    \label{tab:Segmentationtestdev}
    \begin{tabular}{|m{0.8em}|c||c|c|c|c|c|c|} \hline
    &Method&AP&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&$\mathrm{AP_{S}}$ &$\mathrm{AP_{M}}$&$\mathrm{AP_{L}}$\\ \hline 
    \multirow{6}{*}{\rotatebox{90}{w/o DCN}}&Polar Mask \cite{polarmask}&$32.1$&$53.7$&$33.1$&$14.7$&$33.8$&$45.3$\\ 
%    D-SOLO \cite{solo}&$38.4$&$59.6$&$41.1$&$16.8$&$41.5$&$54.6$\\ 
%    &Blend Mask \cite{blendmask}&$39.6$&$\mathbf{61.6}$&$42.6$&$\mathbf{22.4}$&$42.2$&$51.4$\\
    &Mask R-CNN \cite{tensormask} &$38.3$&$61.2$&$40.8$&$18.2$&$40.6$&$54.1$ \\
    &SOLOv2 \cite{solov2}&$39.7$&$60.7$&$42.9$&$17.3$&$42.9$&$\mathbf{57.4}$\\
    &Center Mask \cite{centermask} &$39.8$&--&--&$21.7$&$42.5$&$52.0$\\  
    &BCNet \cite{BCNet}&$39.8$&$61.5$&$43.1$&$22.7$&$42.4$&$51.1$\\ \cline{2-8}
%    &RS-SOLOv2 (Ours)&$\mathbf{40.2}$&$61.5$&$\mathbf{43.3}$&$17.4$&$\mathbf{43.3}$&$\mathbf{58.5}$ \\ 
    &RS-Mask R-CNN (Ours)&$40.6$&$62.8$&$43.9$&$22.8$&$43.6$&$52.8$ \\
    &RS-Mask R-CNN+ (Ours)&$\mathbf{42.0}$&$\mathbf{64.8}$&$\mathbf{45.6}$&$\mathbf{24.2}$&$\mathbf{45.1}$&$54.6$ \\ \hline
    \hhline{========}
    \multirow{5}{*}{\rotatebox{90}{w DCN}}&Mask-scoring R-CNN \cite{maskscoring}&$39.6$&$60.7$&$43.1$&$18.8$&$41.5$&$56.2$\\
    &BlendMask \cite{blendmask}&$41.3$&$63.1$&$44.6$&$22.7$&$44.1$&$54.5$\\
    &SOLOv2 \cite{solov2}&$41.7$&$63.2$&$45.1$&$18.0$&$45.0$&$\mathbf{61.6}$\\ \cline{2-8}
    &RS-Mask R-CNN+ (Ours)&$\mathbf{43.9}$&$\mathbf{67.1}$&$\mathbf{47.6}$&$\mathbf{25.6}$&$\mathbf{47.0}$&$57.8$\\ \cline{2-8}
    &RS-Mask R-CNN+* (Ours)&$44.8$&$68.4$&$48.6$&$27.1$&$47.9$&$58.3$\\ 
    %\cline{2-8} &RS-Mask R-CNN+$^*$ (Ours)&$45.3$&$68.6$&$49.4$&$28.5$&$48.4$&$57.4$\\ 
    %\cline{2-8}&RS-Mask R-CNN+ (MS Test)&$\mathbf{?}$&$?$&$\mathbf{?}$&$?$&$\mathbf{?}$&$\mathbf{?}$ \\ 
    \hline
    \end{tabular}
\end{table}

\subsection{Ablation Experiments}
\label{subsec:Ablation}
\textbf{Contribution of the components:} Replacing Focal Loss by RS Loss improves the performance significantly ($1$ AP - Table \ref{tbl:ablation}). Score-based weighting has a minor contribution and value-based task balancing simplifies tuning. 

\begin{table}
 \centering
\setlength{\tabcolsep}{0.25em}
\footnotesize
\caption{Contribution of the components of RS Loss on ATSS. \label{tbl:ablation}} 
\begin{tabular}{|c|c|c|c||c|c|}
\hline
Architecture&RS Loss&score-based w.&task bal.&$\mathrm{AP}$&H\# $\downarrow$\\ \hline
& & & &$38.7$&3\\ \cline{2-6}
ATSS+ResNet50&\checkmark& & &$39.7$&2\\ \cline{2-6}
w.o. aux. head&\checkmark&\checkmark& &$39.8$&2\\  \cline{2-6}
&\checkmark&\checkmark&\checkmark&$39.9$&1\\ \hline
\end{tabular}
\end{table}

\begin{table}
    \centering
\setlength{\tabcolsep}{0.35em}
    \footnotesize
    \caption{Ablation with different degrees of imbalance on different datasets and samplers. Number of negatives (neg) corresponding to a single positive (pos) averaged over the iterations of the first epoch is presented.
    %For each pos. instance (ins.), e.g. anchor, random (rand.) sampler aims to sample 1 neg. instance in RPN and 3 neg. instance in RCNN. With no sampler (none), there is no desired instance rate, i.e. not available - N/A. Note that when rand. sampler cannot find enough pos., the batch is padded with neg.; accordingly, actual instance rate presents number of neg. instances for each pos. instance after padding. Also, since we use class-wise binary classifiers on RCNN; each neg. instance has $O$ neg. tasks, and each pos. instance has $1$ pos. and $O-1$ neg. tasks where $O$ is the number of dataset classes (see Sec. 3.1 of Tan et al. [C] for details). Using this, actual class rate (underlined) presents the actual imbalance rate in the input of RS Loss as number of neg. tasks for a pos. task. 
    Quantitatively, pos:neg ratio varies between 1:7 to 1:10470. RS Loss successfully trains different degrees of imbalance without tuning (Tables \ref{tab:TwoStage} and \ref{tbl:LVIS}). Details: Appendix \ref{sec:Experiments_supp}}
    \label{tab:SamplingEffect}
    \begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
    \multirow{2}{*}{Dataset}&\multicolumn{2}{|c|}{Sampler}&\multicolumn{2}{|c|}{Desired Neg \#}&\multicolumn{2}{|c|}{Actual Neg \#}&\multirow{2}{*}{$\mathrm{AP}$}\\ \cline{2-7}
    &RPN&R-CNN&RPN&R-CNN&RPN&R-CNN&\\ \hline
    \multirow{3}{*}{COCO}&Random&Random&1&3&7&702& 38.5\\ 
    &None&Random&1&N/A&6676&702&39.3\\
    &None&None&N/A&N/A&6676&1142&39.6 \\     \hline
    LVIS&None&None&N/A&N/A&3487&10470&25.2 \\     \hline
    \end{tabular}
\end{table}

\comment{
\begin{table}
    \centering
    \footnotesize
    \caption{RS Loss is robust to class imbalance. It successfully trains Faster R-CNN with both relatively balanced (``Random'' sampling) and severely imbalanced (``None'' in the table) data. Numbers in parentheses show positive to negative ratio of sampled examples.}
    \label{tab:SamplingEffect}
    \begin{tabular}{|c|c||c|c|c|} \hline
    RPN&R-CNN&AP&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$\\ \hline 
    Random (1:1)&Random (1:3)&$38.5$&$58.5$&$41.5$ \\ 
    None&Random (1:3)&$39.3$&$\mathbf{59.6}$&$42.3$\\
    None&None&$\mathbf{39.6}$&$59.5$&$\mathbf{43.0}$ \\ \hline
    \end{tabular}
\end{table}
}

\textbf{Robustness to imbalance:} Without tuning, RS Loss can train models with very different imbalance levels successfully (Table \ref{tab:SamplingEffect}): Our RS Loss (i) yields $38.5$ AP on COCO with the standard random samplers (i.e. data is relatively balanced especially for RPN), (ii) utilizes more data when the samplers are removed, resulting in $\smallsim1$ AP gain ($38.5$ to $39.6$ AP), and (iii) outperforms all counterparts on the long-tailed LVIS dataset (c.f. Table \ref{tbl:LVIS}), where the imbalance is extreme for R-CNN (pos:neg ratio is $1:10470$ - Table \ref{tab:SamplingEffect}). Appendix \ref{sec:Experiments_supp} presents detailed discussion. 

% Moreover, while we train models with different distributions, unlike score-based losses (i.e. Focal Loss \cite{FocalLoss}, QFL \cite{GFL}), we do not tune the bias terms in the last layer of the classification head to prevent destabilization of the training due to large loss value originating from negatives, which is shown to be important for score-based loss functions \cite{SamplingHeuristics}.

\textbf{Contribution of the sorting error:} To see the contribution of our additional sorting error, during training, we track Spearman's ranking correlation coefficient ($\rho$) between IoUs and classification scores, as an indicator of the sorting quality, with and without our additional sorting error (see Eq. \ref{eq:RSLoss}-\ref{eq:RSTarget}). As hypothesized, using sorting error improves sorting quality, $\rho$, averaged over all/last 100 iterations, from $0.38/0.42$ to $0.42/0.47$ for RS-R-CNN.

\textbf{Effect on Efficiency:} On average, one training iteration of RS Loss takes around $1.5 \times$ longer than score-based losses. See Appendix \ref{sec:Experiments_supp} for more discussion on the effect of RS Loss on training and inference time.


==> RankSort (arXiv)/sections/7.Conclusion.tex <==
\section{Conclusion}
In this paper, we proposed RS Loss as a ranking-based loss function to train object detectors and instance segmentation methods. Unlike existing ranking-based losses, which aim to rank positives above negatives, our RS Loss also sorts positives wrt. their localisation qualities, which is consistent with NMS and the performance measure, AP. With RS Loss, we  employed a simple, loss-value-based, tuning-free heuristic to balance all heads in the visual detectors. As a result, we showed on seven diverse visual detectors that RS Loss both consistently improves performance and significantly simplifies the training pipeline.
%We note that while our loss design presents a strong baseline wrt. performance, it is only validated on the common SOTA baseline ATSS, and the performance of other detectors may be improved further by a grid search or better task-balancing methods. Also, similar to other ranking-based losses \cite{APLoss}, the time and space complexity is quadratic since of RS Loss considers the ranking between each pair, and thus, training takes $\sim 1.5 \times$ longer on average compared to standard training. Nevertheless, we demonstrate on several detectors that one can achieve better performance than its score based alternatives using RS Loss only by tuning the learning rate and significantly simplifying training.
